CROCODIL: Cross-Model Code Editing with LLMs

Large language models (LLMs) have become ubiquitous tools for code generation and editing. However, development teams often use multiple LLM assistants. Different developers may prefer different models, and individual developers may switch between models across different coding sessions. Because of this, the edits any one model makes are frequently applied to foreign code originally generated by another model. These LLMs are often trained on different datasets, and as a result have different stylistic preferences. Do LLMs behave differently when they edit foreign code originally written by a different LLM with a different coding style? We find that models tend to make more, and often excessive, edits on foreign code. We introduce CROCODIL (Cross-model Code Editing with LLMs), a post-training framework for reducing excessive edits while preserving functional correctness. CROCODIL's similarity reward penalizes large changes, while its execution reward scores build and test success. We use the product of these two rewards to encourage the policy to decrease the edit size without decreasing the edit task success rate. CROCODIL is available at https://github.com/EngineeringSoftware/Crocodil.

==> defs/defs-code.tex <==
\definecolor{gray}{RGB}{211,211,211}
\newcommand{\jbasicstyle}{\small\sffamily}
\newcommand{\textcode}[1]{{#1}}
\newcommand{\jnumberstyle}{\scriptsize}
\newcommand{\Hilight}{\makebox[0pt][l]{\color{gray}\rule[-3pt]{0.80\linewidth}{9pt}}}

\lstdefinelanguage{pseudo}
{
  morekeywords={},
  keywordstyle=\bfseries,
  lineskip=-0.1em,
  numbers=left,
  numberstyle=\jnumberstyle,
  numbersep=4pt,
  basicstyle=\jbasicstyle,
  breaklines=true,
  breakautoindent=true,
  tabsize=2,
  columns=fullflexible,
  morecomment=*[l][\textsl]{//},
  mathescape=true,
  xleftmargin=10pt,
}

\lstdefinelanguage{todo-comment}
{
  morekeywords={},
  keywordstyle=\bfseries,
  lineskip=-0.1em,
  numbers=none,
  basicstyle=\jbasicstyle,
  breaklines=true,
  breakautoindent=true,
  tabsize=2,
  columns=fullflexible,
  morecomment=*[l][\textsl]{//},
  mathescape=true,
  xleftmargin=-10pt,
}

\lstdefinelanguage{java-pretty}
{
  language=java,
  numbers=left,
  basicstyle=\scriptsize\ttfamily,
  numberstyle=\scriptsize,
  breaklines=true,
  columns=fullflexible,
  xleftmargin=16pt,
  showstringspaces=false,
}

\definecolor{rust-keyword}{rgb}{0.74, 0.2, 0.64}
\definecolor{rust-modifier}{rgb}{0.2, 0.2, 0.6}
\definecolor{rust-type}{rgb}{0.0, 0.42, 0.24}
\definecolor{rust-fn}{rgb}{0.25, 0.5, 0.35}
\definecolor{rust-comment}{rgb}{0.45, 0.45, 0.45}
\definecolor{rust-string}{rgb}{0.65, 0.16, 0.16}
\definecolor{gitgreen}{rgb}{0.0, 0.5, 0.0}
\definecolor{gitred}{rgb}{0.7, 0.0, 0.0}

\lstdefinelanguage{rust-pretty}
{
  morekeywords=[1]{if, else, while, loop, for, match, break, continue, return, in, as, where},
  keywordstyle=[1]\color{rust-keyword}\bfseries,
  morekeywords=[2]{pub, mut, ref, const, static, let, move, async, await, unsafe, crate, use, mod, super, self, Self},
  keywordstyle=[2]\color{rust-modifier}\bfseries,
  morekeywords=[3]{bool, char, i8, i16, i32, i64, i128, u8, u16, u32, u64, u128, usize, isize, f32, f64, str, String, Vec, Option, Result, Box, Cursor},
  keywordstyle=[3]\color{rust-type}\bfseries,
  morekeywords=[4]{fn, struct, enum, trait, impl, type, dyn, Some, None, Ok, Err, true, false},
  keywordstyle=[4]\color{rust-fn},
  morecomment=[l]{//},
  commentstyle=\color{rust-comment}\itshape,
  morestring=[b]",
  stringstyle=\color{rust-string},
  numbers=left,
  basicstyle=\scriptsize\ttfamily,
  numberstyle=\scriptsize,
  breaklines=true,
  columns=fullflexible,
  xleftmargin=14pt,
  tabsize=2,
  showstringspaces=false,
  keepspaces=true,
}

\lstdefinelanguage{rust-diff}
{
  language=rust-pretty,
  morecomment=[f][\color{gitgreen}][0]{+},
  morecomment=[f][\color{gitred}][0]{-},
  escapeinside={(*@}{@*)},
  showstringspaces=false,
  keepspaces=true,
  breaklines=true,
}

\lstset{escapeinside={(*@}{@*)}}

\lstdefinestyle{ContextSnippet}{
  basicstyle=\footnotesize\ttfamily,
  breaklines=true,
  breakautoindent=true,
  breakatwhitespace=false,
  columns=fullflexible,
  keepspaces=true,
  showstringspaces=false,
  xleftmargin=4pt,
}


==> defs/defs-logic.tex <==
\newcommand{\ltrue}{\top}
\newcommand{\lfalse}{\bot}

\newcommand{\limply}{\rightarrow}
\newcommand{\liff}{\leftrightarrow}
\newcommand{\lcofactor}{\downarrow}

\newcommand{\llimply}{\Rightarrow}
\newcommand{\lliff}{\Leftrightarrow}
\newcommand{\lsat}{\vDash}
\newcommand{\lnsat}{\nvDash}

\newcommand{\lqall}[1]{\forall #1.~}
\newcommand{\lqexist}[1]{\exists #1.~}
\newcommand{\lqallOnly}[1]{\forall #1 }
\newcommand{\lqexistOnly}[1]{\exists #1 }

\newcommand{\lAnd}[1]{\bigwedge_{\substack{#1}}}
\newcommand{\lOr}[1]{\bigvee_{\substack{#1}}}

\newcommand{\set}[1]{\{#1\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\tuple}[1]{\langle#1\rangle}
\newcommand{\Tuple}[1]{\left\langle#1\right\rangle}

\newcommand{\sunion}{\cup}
\newcommand{\sinter}{\cap}


==> tables/corpus_attrition_after_table.tex <==
% The second half of the funnel, from the \reimplementation on: one row per
% filter, in pipeline order, and one column per \rewriter, since each now has
% its own count. Measured 211.5pt against \columnwidth 219.1pt: five stacked
% model headers take 163.5pt, so the filter name sits in a 42pt paragraph
% column that wraps and hyphenates rather than in a fixed stack.
\begin{table}[h]
  \centering
  \small
  \setlength{\tabcolsep}{3pt}
  % siunitx ignores the surrounding font by default, so \textbf{\num{...}}
  % prints roman. Scoped to this table, which is the only one that bolds a
  % \num cell.
  \sisetup{detect-weight=true, detect-family=true}
  \begin{tabular}{@{}>{\raggedright\arraybackslash}p{42pt}ccccc@{}}
    \toprule
     & \textbf{\UseMacro{TCol-qwen}} & \textbf{\UseMacro{TCol-gpto}} & \textbf{\UseMacro{TCol-olmos}} & \textbf{\UseMacro{TCol-olmol}} & \textbf{\UseMacro{TCol-haiku}} \\
    \midrule
    Pass \reimplementation test & \num{\UseMacro{edit-filter-eval-rust-repos-qwen-wide-passing}} & \num{\UseMacro{edit-filter-eval-rust-repos-gpt-wide-passing}} & \num{\UseMacro{edit-filter-eval-rust-repos-olmo7b-wide-passing}} & \num{\UseMacro{edit-filter-eval-rust-repos-olmo32b-wide-passing}} & \num{\UseMacro{edit-filter-eval-rust-repos-haiku-wide-passing}} \\
    \midrule
    Overlap below 50\% & \num{\UseMacro{edit-filter-eval-rust-repos-qwen-wide-after-overlap}} & \num{\UseMacro{edit-filter-eval-rust-repos-gpt-wide-after-overlap}} & \num{\UseMacro{edit-filter-eval-rust-repos-olmo7b-wide-after-overlap}} & \num{\UseMacro{edit-filter-eval-rust-repos-olmo32b-wide-after-overlap}} & \num{\UseMacro{edit-filter-eval-rust-repos-haiku-wide-after-overlap}} \\
    \midrule
    Fail edit test & \num{\UseMacro{edit-filter-eval-rust-repos-qwen-after-presolved}} & \num{\UseMacro{edit-filter-eval-rust-repos-gpt-after-presolved}} & \num{\UseMacro{edit-filter-eval-rust-repos-olmo7b-after-presolved}} & \num{\UseMacro{edit-filter-eval-rust-repos-olmo32b-after-presolved}} & \num{\UseMacro{edit-filter-eval-rust-repos-haiku-after-presolved}} \\
    \midrule
    \IDPRdesc available & \textbf{\num{\UseMacro{edit-filter-eval-rust-repos-qwen-after-nodesc}}} & \textbf{\num{\UseMacro{edit-filter-eval-rust-repos-gpt-after-nodesc}}} & \textbf{\num{\UseMacro{edit-filter-eval-rust-repos-olmo7b-after-nodesc}}} & \textbf{\num{\UseMacro{edit-filter-eval-rust-repos-olmo32b-after-nodesc}}} & \textbf{\num{\UseMacro{edit-filter-eval-rust-repos-haiku-after-nodesc}}} \\
    \bottomrule
  \end{tabular}
  \caption{\UseMacro{TCap-corpus-attrition-after}}
  \label{tab:corpus-attrition-after}
\end{table}


==> tables/corpus_attrition_before_table.tex <==
% The first half of the funnel, before the \reimplementation: one row per
% filter, in pipeline order. Shared across \rewriters, since every one of them is asked
% for the same functions, so a single Functions column carries all five.
% Measured 145.4pt against \columnwidth 219.1pt.
\begin{table}[h]
  \centering
  \small
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{@{}lc@{}}
    \toprule
    \textbf{Filter} & \textbf{Functions} \\
    \midrule
    \PR and function-level filters & \num{\UseMacro{corpus-eval-rust-repos-split-functions}} \\
    README available & \num{\UseMacro{corpus-eval-rust-repos-readme-functions}} \\
    Tests available & \num{\UseMacro{corpus-eval-rust-repos-pretests-functions}} \\
    \IDCallsites available & \num{\UseMacro{corpus-eval-rust-repos-target-after-callsites}} \\
    \IDFuncdesc available & \num{\UseMacro{corpus-eval-rust-repos-draft-target-functions}} \\
    \bottomrule
  \end{tabular}
  \caption{\UseMacro{TCap-corpus-attrition-before}}
  \label{tab:corpus-attrition-before}
\end{table}


==> tables/pr_edit_pass_rate_pivot_table.tex <==
\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l c c c c c}
\toprule
\multirow{2}{*}{\textbf{Impl.}} & \multicolumn{5}{c}{\textbf{Editor}} \\
\cmidrule(lr){2-6}
 & \textbf{\UseMacro{TCol-qwen}} & \textbf{\UseMacro{TCol-gpto}} & \textbf{\UseMacro{TCol-olmos}} & \textbf{\UseMacro{TCol-olmol}} & \textbf{\UseMacro{TCol-haiku}} \\
\midrule
\textbf{\UseMacro{TColInline-qwen}} & \UseMacro{fig-pr-edit-pass-rate-pivot-qwen3.5-thinking:35b-a3b-q4-k-m-qwen3.5-thinking:35b-a3b-q4-k-m-tests} & \UseMacro{fig-pr-edit-pass-rate-pivot-qwen3.5-thinking:35b-a3b-q4-k-m-gpt-oss:20b-q4-k-m-tests} & \UseMacro{fig-pr-edit-pass-rate-pivot-qwen3.5-thinking:35b-a3b-q4-k-m-olmo3-thinking:7b.think-q4-k-m-tests} & \UseMacro{fig-pr-edit-pass-rate-pivot-qwen3.5-thinking:35b-a3b-q4-k-m-olmo3.1-thinking:32b.think-q4-k-m-tests} & \textbf{\UseMacro{fig-pr-edit-pass-rate-pivot-qwen3.5-thinking:35b-a3b-q4-k-m-claude-haiku-4-5-tests}} \\
\textbf{\UseMacro{TColInline-gpto}} & \UseMacro{fig-pr-edit-pass-rate-pivot-gpt-oss:20b-q4-k-m-qwen3.5-thinking:35b-a3b-q4-k-m-tests} & \UseMacro{fig-pr-edit-pass-rate-pivot-gpt-oss:20b-q4-k-m-gpt-oss:20b-q4-k-m-tests} & \UseMacro{fig-pr-edit-pass-rate-pivot-gpt-oss:20b-q4-k-m-olmo3-thinking:7b.think-q4-k-m-tests} & \UseMacro{fig-pr-edit-pass-rate-pivot-gpt-oss:20b-q4-k-m-olmo3.1-thinking:32b.think-q4-k-m-tests} & \UseMacro{fig-pr-edit-pass-rate-pivot-gpt-oss:20b-q4-k-m-claude-haiku-4-5-tests} \\
\textbf{\UseMacro{TColInline-olmos}} & \UseMacro{fig-pr-edit-pass-rate-pivot-olmo3-thinking:7b.think-q4-k-m-qwen3.5-thinking:35b-a3b-q4-k-m-tests} & \UseMacro{fig-pr-edit-pass-rate-pivot-olmo3-thinking:7b.think-q4-k-m-gpt-oss:20b-q4-k-m-tests} & \textbf{\UseMacro{fig-pr-edit-pass-rate-pivot-olmo3-thinking:7b.think-q4-k-m-olmo3-thinking:7b.think-q4-k-m-tests}} & \UseMacro{fig-pr-edit-pass-rate-pivot-olmo3-thinking:7b.think-q4-k-m-olmo3.1-thinking:32b.think-q4-k-m-tests} & \UseMacro{fig-pr-edit-pass-rate-pivot-olmo3-thinking:7b.think-q4-k-m-claude-haiku-4-5-tests} \\
\textbf{\UseMacro{TColInline-olmol}} & \textbf{\UseMacro{fig-pr-edit-pass-rate-pivot-olmo3.1-thinking:32b.think-q4-k-m-qwen3.5-thinking:35b-a3b-q4-k-m-tests}} & \textbf{\UseMacro{fig-pr-edit-pass-rate-pivot-olmo3.1-thinking:32b.think-q4-k-m-gpt-oss:20b-q4-k-m-tests}} & \UseMacro{fig-pr-edit-pass-rate-pivot-olmo3.1-thinking:32b.think-q4-k-m-olmo3-thinking:7b.think-q4-k-m-tests} & \textbf{\UseMacro{fig-pr-edit-pass-rate-pivot-olmo3.1-thinking:32b.think-q4-k-m-olmo3.1-thinking:32b.think-q4-k-m-tests}} & \UseMacro{fig-pr-edit-pass-rate-pivot-olmo3.1-thinking:32b.think-q4-k-m-claude-haiku-4-5-tests} \\
\textbf{\UseMacro{TColInline-haiku}} & \UseMacro{fig-pr-edit-pass-rate-pivot-claude-haiku-4-5-qwen3.5-thinking:35b-a3b-q4-k-m-tests} & \UseMacro{fig-pr-edit-pass-rate-pivot-claude-haiku-4-5-gpt-oss:20b-q4-k-m-tests} & \UseMacro{fig-pr-edit-pass-rate-pivot-claude-haiku-4-5-olmo3-thinking:7b.think-q4-k-m-tests} & \UseMacro{fig-pr-edit-pass-rate-pivot-claude-haiku-4-5-olmo3.1-thinking:32b.think-q4-k-m-tests} & \UseMacro{fig-pr-edit-pass-rate-pivot-claude-haiku-4-5-claude-haiku-4-5-tests} \\
\bottomrule
\end{tabular}
\caption{\UseMacro{TCap-pr-edit-pass-rate-pivot}}
\label{tab:pr-edit-pass-rate-pivot}
\end{table}

==> tables/pr_lev_minmax_norm_pivot_rewrite_char_table.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l c c c c c}
\toprule
\multirow{2}{*}{\textbf{Impl.}} & \multicolumn{5}{c}{\textbf{Editor}} \\
\cmidrule(lr){2-6}
 & \textbf{\UseMacro{TCol-qwen}} & \textbf{\UseMacro{TCol-gpto}} & \textbf{\UseMacro{TCol-olmos}} & \textbf{\UseMacro{TCol-olmol}} & \textbf{\UseMacro{TCol-haiku}} \\
\midrule
\UseMacro{TColInline-qwen} & \textbf{\UseMacro{fig-pr-lev-minmax-norm-pivot-all-qwen3.5-thinking:35b-a3b-q4-k-m-qwen3.5-thinking:35b-a3b-q4-k-m-lev-char}} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-qwen3.5-thinking:35b-a3b-q4-k-m-gpt-oss:20b-q4-k-m-lev-char} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-qwen3.5-thinking:35b-a3b-q4-k-m-olmo3-thinking:7b.think-q4-k-m-lev-char} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-qwen3.5-thinking:35b-a3b-q4-k-m-olmo3.1-thinking:32b.think-q4-k-m-lev-char} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-qwen3.5-thinking:35b-a3b-q4-k-m-claude-haiku-4-5-lev-char} \\
\UseMacro{TColInline-gpto} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-gpt-oss:20b-q4-k-m-qwen3.5-thinking:35b-a3b-q4-k-m-lev-char} & \textbf{\UseMacro{fig-pr-lev-minmax-norm-pivot-all-gpt-oss:20b-q4-k-m-gpt-oss:20b-q4-k-m-lev-char}} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-gpt-oss:20b-q4-k-m-olmo3-thinking:7b.think-q4-k-m-lev-char} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-gpt-oss:20b-q4-k-m-olmo3.1-thinking:32b.think-q4-k-m-lev-char} & \textbf{\UseMacro{fig-pr-lev-minmax-norm-pivot-all-gpt-oss:20b-q4-k-m-claude-haiku-4-5-lev-char}} \\
\UseMacro{TColInline-olmos} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-olmo3-thinking:7b.think-q4-k-m-qwen3.5-thinking:35b-a3b-q4-k-m-lev-char} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-olmo3-thinking:7b.think-q4-k-m-gpt-oss:20b-q4-k-m-lev-char} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-olmo3-thinking:7b.think-q4-k-m-olmo3-thinking:7b.think-q4-k-m-lev-char} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-olmo3-thinking:7b.think-q4-k-m-olmo3.1-thinking:32b.think-q4-k-m-lev-char} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-olmo3-thinking:7b.think-q4-k-m-claude-haiku-4-5-lev-char} \\
\UseMacro{TColInline-olmol} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-olmo3.1-thinking:32b.think-q4-k-m-qwen3.5-thinking:35b-a3b-q4-k-m-lev-char} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-olmo3.1-thinking:32b.think-q4-k-m-gpt-oss:20b-q4-k-m-lev-char} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-olmo3.1-thinking:32b.think-q4-k-m-olmo3-thinking:7b.think-q4-k-m-lev-char} & \textbf{\UseMacro{fig-pr-lev-minmax-norm-pivot-all-olmo3.1-thinking:32b.think-q4-k-m-olmo3.1-thinking:32b.think-q4-k-m-lev-char}} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-olmo3.1-thinking:32b.think-q4-k-m-claude-haiku-4-5-lev-char} \\
\UseMacro{TColInline-haiku} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-claude-haiku-4-5-qwen3.5-thinking:35b-a3b-q4-k-m-lev-char} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-claude-haiku-4-5-gpt-oss:20b-q4-k-m-lev-char} & \textbf{\UseMacro{fig-pr-lev-minmax-norm-pivot-all-claude-haiku-4-5-olmo3-thinking:7b.think-q4-k-m-lev-char}} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-claude-haiku-4-5-olmo3.1-thinking:32b.think-q4-k-m-lev-char} & \UseMacro{fig-pr-lev-minmax-norm-pivot-all-claude-haiku-4-5-claude-haiku-4-5-lev-char} \\
\bottomrule
\end{tabular}
\caption{\UseMacro{TCap-pr-lev-minmax-norm-pivot-rewrite-char}}
\label{tab:pr-lev-minmax-norm-pivot-rewrite-char}
\end{table}

==> tables/pr_lev_selfcross_mwu_table.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l c c c c c}
\toprule
\multirow{2}{*}{\textbf{Impl.}} & \multicolumn{5}{c}{\textbf{Editor}} \\
\cmidrule(lr){2-6}
 & \textbf{\UseMacro{TCol-qwen}} & \textbf{\UseMacro{TCol-gpto}} & \textbf{\UseMacro{TCol-olmos}} & \textbf{\UseMacro{TCol-olmol}} & \textbf{\UseMacro{TCol-haiku}} \\
\midrule
\UseMacro{TColInline-qwen} & -- & \UseMacro{fig-pr-lev-selfcross-mwu-qwen3.5-thinking:35b-a3b-q4-k-m-gpt-oss:20b-q4-k-m-p}\UseMacro{fig-pr-lev-selfcross-mwu-qwen3.5-thinking:35b-a3b-q4-k-m-gpt-oss:20b-q4-k-m-stars} & \UseMacro{fig-pr-lev-selfcross-mwu-qwen3.5-thinking:35b-a3b-q4-k-m-olmo3-thinking:7b.think-q4-k-m-p}\UseMacro{fig-pr-lev-selfcross-mwu-qwen3.5-thinking:35b-a3b-q4-k-m-olmo3-thinking:7b.think-q4-k-m-stars} & \UseMacro{fig-pr-lev-selfcross-mwu-qwen3.5-thinking:35b-a3b-q4-k-m-olmo3.1-thinking:32b.think-q4-k-m-p}\UseMacro{fig-pr-lev-selfcross-mwu-qwen3.5-thinking:35b-a3b-q4-k-m-olmo3.1-thinking:32b.think-q4-k-m-stars} & \UseMacro{fig-pr-lev-selfcross-mwu-qwen3.5-thinking:35b-a3b-q4-k-m-claude-haiku-4-5-p}\UseMacro{fig-pr-lev-selfcross-mwu-qwen3.5-thinking:35b-a3b-q4-k-m-claude-haiku-4-5-stars} \\
\UseMacro{TColInline-gpto} & \UseMacro{fig-pr-lev-selfcross-mwu-gpt-oss:20b-q4-k-m-qwen3.5-thinking:35b-a3b-q4-k-m-p}\UseMacro{fig-pr-lev-selfcross-mwu-gpt-oss:20b-q4-k-m-qwen3.5-thinking:35b-a3b-q4-k-m-stars} & -- & \UseMacro{fig-pr-lev-selfcross-mwu-gpt-oss:20b-q4-k-m-olmo3-thinking:7b.think-q4-k-m-p}\UseMacro{fig-pr-lev-selfcross-mwu-gpt-oss:20b-q4-k-m-olmo3-thinking:7b.think-q4-k-m-stars} & \UseMacro{fig-pr-lev-selfcross-mwu-gpt-oss:20b-q4-k-m-olmo3.1-thinking:32b.think-q4-k-m-p}\UseMacro{fig-pr-lev-selfcross-mwu-gpt-oss:20b-q4-k-m-olmo3.1-thinking:32b.think-q4-k-m-stars} & \UseMacro{fig-pr-lev-selfcross-mwu-gpt-oss:20b-q4-k-m-claude-haiku-4-5-p}\UseMacro{fig-pr-lev-selfcross-mwu-gpt-oss:20b-q4-k-m-claude-haiku-4-5-stars} \\
\UseMacro{TColInline-olmos} & \UseMacro{fig-pr-lev-selfcross-mwu-olmo3-thinking:7b.think-q4-k-m-qwen3.5-thinking:35b-a3b-q4-k-m-p}\UseMacro{fig-pr-lev-selfcross-mwu-olmo3-thinking:7b.think-q4-k-m-qwen3.5-thinking:35b-a3b-q4-k-m-stars} & \UseMacro{fig-pr-lev-selfcross-mwu-olmo3-thinking:7b.think-q4-k-m-gpt-oss:20b-q4-k-m-p}\UseMacro{fig-pr-lev-selfcross-mwu-olmo3-thinking:7b.think-q4-k-m-gpt-oss:20b-q4-k-m-stars} & -- & \UseMacro{fig-pr-lev-selfcross-mwu-olmo3-thinking:7b.think-q4-k-m-olmo3.1-thinking:32b.think-q4-k-m-p}\UseMacro{fig-pr-lev-selfcross-mwu-olmo3-thinking:7b.think-q4-k-m-olmo3.1-thinking:32b.think-q4-k-m-stars} & \UseMacro{fig-pr-lev-selfcross-mwu-olmo3-thinking:7b.think-q4-k-m-claude-haiku-4-5-p}\UseMacro{fig-pr-lev-selfcross-mwu-olmo3-thinking:7b.think-q4-k-m-claude-haiku-4-5-stars} \\
\UseMacro{TColInline-olmol} & \UseMacro{fig-pr-lev-selfcross-mwu-olmo3.1-thinking:32b.think-q4-k-m-qwen3.5-thinking:35b-a3b-q4-k-m-p}\UseMacro{fig-pr-lev-selfcross-mwu-olmo3.1-thinking:32b.think-q4-k-m-qwen3.5-thinking:35b-a3b-q4-k-m-stars} & \UseMacro{fig-pr-lev-selfcross-mwu-olmo3.1-thinking:32b.think-q4-k-m-gpt-oss:20b-q4-k-m-p}\UseMacro{fig-pr-lev-selfcross-mwu-olmo3.1-thinking:32b.think-q4-k-m-gpt-oss:20b-q4-k-m-stars} & \UseMacro{fig-pr-lev-selfcross-mwu-olmo3.1-thinking:32b.think-q4-k-m-olmo3-thinking:7b.think-q4-k-m-p}\UseMacro{fig-pr-lev-selfcross-mwu-olmo3.1-thinking:32b.think-q4-k-m-olmo3-thinking:7b.think-q4-k-m-stars} & -- & \UseMacro{fig-pr-lev-selfcross-mwu-olmo3.1-thinking:32b.think-q4-k-m-claude-haiku-4-5-p}\UseMacro{fig-pr-lev-selfcross-mwu-olmo3.1-thinking:32b.think-q4-k-m-claude-haiku-4-5-stars} \\
\UseMacro{TColInline-haiku} & \UseMacro{fig-pr-lev-selfcross-mwu-claude-haiku-4-5-qwen3.5-thinking:35b-a3b-q4-k-m-p}\UseMacro{fig-pr-lev-selfcross-mwu-claude-haiku-4-5-qwen3.5-thinking:35b-a3b-q4-k-m-stars} & \UseMacro{fig-pr-lev-selfcross-mwu-claude-haiku-4-5-gpt-oss:20b-q4-k-m-p}\UseMacro{fig-pr-lev-selfcross-mwu-claude-haiku-4-5-gpt-oss:20b-q4-k-m-stars} & \UseMacro{fig-pr-lev-selfcross-mwu-claude-haiku-4-5-olmo3-thinking:7b.think-q4-k-m-p}\UseMacro{fig-pr-lev-selfcross-mwu-claude-haiku-4-5-olmo3-thinking:7b.think-q4-k-m-stars} & \UseMacro{fig-pr-lev-selfcross-mwu-claude-haiku-4-5-olmo3.1-thinking:32b.think-q4-k-m-p}\UseMacro{fig-pr-lev-selfcross-mwu-claude-haiku-4-5-olmo3.1-thinking:32b.think-q4-k-m-stars} & -- \\
\bottomrule
\end{tabular}
\caption{\UseMacro{TCap-pr-lev-selfcross-mwu}}
\label{tab:pr-lev-selfcross-mwu}
\end{table}

==> tables/verl_lev_normfull_rustfmt_table.tex <==
% Hand-written body, rebuilt by scratchpad/build_combined.py. The
% min-max normalized half of the appendix edit-size pair. Four column groups,
% All tasks plus the three equal-outcome populations, at character and
% line granularity. Raw and normalized are two tables rather than one:
% together they are 17 columns and measured 80.5pt past \textwidth.
% A baseline that does not define a group prints ``--'' there. Every
% cell is bolded when it wins its group: \SmallestBoldSafe against the
% other two rows under All tasks, \SmallerBoldSafe against the one peer
% elsewhere. The trailing \UseMacro{...-small} is a dagger when the cell
% averages at most _VERL_SMALL_POPULATION_MARK tasks. Set at \small with
% no \resizebox, like every other table in the paper: the stacked group
% headers are what make the columns fit.
\begin{table*}[h]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l cc cc cc cc}
\toprule
\multirow{2}{*}{\shortstack[l]{\textbf{Implementor} \\ \quad\textbf{Editor}}} & \multicolumn{2}{c}{\shortstack{\textbf{All} \\ \textbf{\tasks}}} & \multicolumn{2}{c}{\shortstack{\textbf{Base \&} \\ \textbf{Strict pass}}} & \multicolumn{2}{c}{\shortstack{\textbf{Base \&} \\ \textbf{RL pass}}} & \multicolumn{2}{c}{\shortstack{\textbf{Strict \&} \\ \textbf{RL pass}}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
 & \textbf{Chars} & \textbf{Lines} & \textbf{Chars} & \textbf{Lines} & \textbf{Chars} & \textbf{Lines} & \textbf{Chars} & \textbf{Lines} \\
\midrule
\multicolumn{9}{@{}l}{\textbf{\qwen}} \\
\quad \baselabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-qwen-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-qwen-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-qwen-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-qwen-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-qwen-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-qwen-lev-line}} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-base-qwen-lev-char}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-prompt-qwen-lev-char}}\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-qwen-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-base-qwen-lev-line}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-prompt-qwen-lev-line}}\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-qwen-lev-line-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-base-qwen-lev-char}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-rl-qwen-lev-char}}\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-qwen-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-base-qwen-lev-line}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-rl-qwen-lev-line}}\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-qwen-lev-line-small} & -- & -- \\
\quad \strictlabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-qwen-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-qwen-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-qwen-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-qwen-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-qwen-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-qwen-lev-line}} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-prompt-qwen-lev-char}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-base-qwen-lev-char}}\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-qwen-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-prompt-qwen-lev-line}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-base-qwen-lev-line}}\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-qwen-lev-line-small} & -- & -- & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-prompt-qwen-lev-char}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-rl-qwen-lev-char}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-qwen-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-prompt-qwen-lev-line}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-rl-qwen-lev-line}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-qwen-lev-line-small} \\
\quad \rllabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-qwen-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-qwen-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-qwen-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-qwen-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-qwen-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-qwen-lev-line}} & -- & -- & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-rl-qwen-lev-char}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-base-qwen-lev-char}}\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-qwen-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-rl-qwen-lev-line}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-base-qwen-lev-line}}\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-qwen-lev-line-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-rl-qwen-lev-char}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-prompt-qwen-lev-char}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-qwen-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-rl-qwen-lev-line}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-prompt-qwen-lev-line}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-qwen-lev-line-small} \\
\midrule
\multicolumn{9}{@{}l}{\textbf{\gpto}} \\
\quad \baselabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-gpt-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-gpt-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-gpt-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-gpt-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-gpt-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-gpt-lev-line}} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-base-gpt-lev-char}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-prompt-gpt-lev-char}}\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-gpt-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-base-gpt-lev-line}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-prompt-gpt-lev-line}}\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-gpt-lev-line-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-base-gpt-lev-char}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-rl-gpt-lev-char}}\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-gpt-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-base-gpt-lev-line}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-rl-gpt-lev-line}}\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-gpt-lev-line-small} & -- & -- \\
\quad \strictlabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-gpt-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-gpt-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-gpt-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-gpt-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-gpt-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-gpt-lev-line}} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-prompt-gpt-lev-char}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-base-gpt-lev-char}}\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-gpt-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-prompt-gpt-lev-line}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-base-gpt-lev-line}}\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-gpt-lev-line-small} & -- & -- & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-prompt-gpt-lev-char}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-rl-gpt-lev-char}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-gpt-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-prompt-gpt-lev-line}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-rl-gpt-lev-line}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-gpt-lev-line-small} \\
\quad \rllabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-gpt-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-gpt-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-gpt-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-gpt-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-gpt-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-gpt-lev-line}} & -- & -- & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-rl-gpt-lev-char}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-base-gpt-lev-char}}\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-gpt-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-rl-gpt-lev-line}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-base-gpt-lev-line}}\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-gpt-lev-line-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-rl-gpt-lev-char}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-prompt-gpt-lev-char}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-gpt-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-rl-gpt-lev-line}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-prompt-gpt-lev-line}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-gpt-lev-line-small} \\
\midrule
\multicolumn{9}{@{}l}{\textbf{\olmos}} \\
\quad \baselabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-olmo7b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-olmo7b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-olmo7b-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-olmo7b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-olmo7b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-olmo7b-lev-line}} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-base-olmo7b-lev-char}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-prompt-olmo7b-lev-char}}\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-olmo7b-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-base-olmo7b-lev-line}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-prompt-olmo7b-lev-line}}\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-olmo7b-lev-line-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-base-olmo7b-lev-char}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-rl-olmo7b-lev-char}}\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-olmo7b-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-base-olmo7b-lev-line}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-rl-olmo7b-lev-line}}\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-olmo7b-lev-line-small} & -- & -- \\
\quad \strictlabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-olmo7b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-olmo7b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-olmo7b-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-olmo7b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-olmo7b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-olmo7b-lev-line}} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-prompt-olmo7b-lev-char}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-base-olmo7b-lev-char}}\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-olmo7b-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-prompt-olmo7b-lev-line}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-base-olmo7b-lev-line}}\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-olmo7b-lev-line-small} & -- & -- & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-prompt-olmo7b-lev-char}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-rl-olmo7b-lev-char}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-olmo7b-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-prompt-olmo7b-lev-line}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-rl-olmo7b-lev-line}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-olmo7b-lev-line-small} \\
\quad \rllabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-olmo7b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-olmo7b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-olmo7b-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-olmo7b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-olmo7b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-olmo7b-lev-line}} & -- & -- & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-rl-olmo7b-lev-char}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-base-olmo7b-lev-char}}\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-olmo7b-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-rl-olmo7b-lev-line}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-base-olmo7b-lev-line}}\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-olmo7b-lev-line-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-rl-olmo7b-lev-char}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-prompt-olmo7b-lev-char}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-olmo7b-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-rl-olmo7b-lev-line}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-prompt-olmo7b-lev-line}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-olmo7b-lev-line-small} \\
\midrule
\multicolumn{9}{@{}l}{\textbf{\olmol}} \\
\quad \baselabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-olmo32b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-olmo32b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-olmo32b-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-olmo32b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-olmo32b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-olmo32b-lev-line}} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-base-olmo32b-lev-char}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-prompt-olmo32b-lev-char}}\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-olmo32b-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-base-olmo32b-lev-line}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-prompt-olmo32b-lev-line}}\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-olmo32b-lev-line-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-base-olmo32b-lev-char}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-rl-olmo32b-lev-char}}\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-olmo32b-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-base-olmo32b-lev-line}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-rl-olmo32b-lev-line}}\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-olmo32b-lev-line-small} & -- & -- \\
\quad \strictlabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-olmo32b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-olmo32b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-olmo32b-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-olmo32b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-olmo32b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-olmo32b-lev-line}} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-prompt-olmo32b-lev-char}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-base-olmo32b-lev-char}}\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-olmo32b-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-prompt-olmo32b-lev-line}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-base-olmo32b-lev-line}}\UseMacro{fig-verl-lev-base-strict-rustfmt-minmax-olmo32b-lev-line-small} & -- & -- & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-prompt-olmo32b-lev-char}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-rl-olmo32b-lev-char}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-olmo32b-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-prompt-olmo32b-lev-line}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-rl-olmo32b-lev-line}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-olmo32b-lev-line-small} \\
\quad \rllabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-olmo32b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-olmo32b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-olmo32b-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-rl-olmo32b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-base-olmo32b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-minmax-prompt-olmo32b-lev-line}} & -- & -- & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-rl-olmo32b-lev-char}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-base-olmo32b-lev-char}}\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-olmo32b-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-rl-olmo32b-lev-line}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-base-olmo32b-lev-line}}\UseMacro{fig-verl-lev-both-pass-rustfmt-minmax-olmo32b-lev-line-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-rl-olmo32b-lev-char}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-prompt-olmo32b-lev-char}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-olmo32b-lev-char-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-rl-olmo32b-lev-line}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-prompt-olmo32b-lev-line}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-minmax-olmo32b-lev-line-small} \\
\bottomrule
\end{tabular}
\caption{\UseMacro{TCap-verl-lev-normfull-rustfmt-eval-rust-repos}}
\label{tab:verl-lev-normfull-rustfmt-eval-rust-repos}
\end{table*}


==> tables/verl_lev_raw_rustfmt_table.tex <==
% Hand-written body, rebuilt by scratchpad/build_combined.py. The
% raw half of the appendix edit-size pair. Four column groups,
% All tasks plus the three equal-outcome populations, at character and
% line granularity. Raw and normalized are two tables rather than one:
% together they are 17 columns and measured 80.5pt past \textwidth.
% A baseline that does not define a group prints ``--'' there. Every
% cell is bolded when it wins its group: \SmallestBoldSafe against the
% other two rows under All tasks, \SmallerBoldSafe against the one peer
% elsewhere. The trailing \UseMacro{...-small} is a dagger when the cell
% averages at most _VERL_SMALL_POPULATION_MARK tasks. Set at \small with
% no \resizebox, like every other table in the paper: the stacked group
% headers are what make the columns fit.
\begin{table*}[h]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l cc cc cc cc}
\toprule
\multirow{2}{*}{\shortstack[l]{\textbf{Implementor} \\ \quad\textbf{Editor}}} & \multicolumn{2}{c}{\shortstack{\textbf{All} \\ \textbf{\tasks}}} & \multicolumn{2}{c}{\shortstack{\textbf{Base \&} \\ \textbf{Strict pass}}} & \multicolumn{2}{c}{\shortstack{\textbf{Base \&} \\ \textbf{RL pass}}} & \multicolumn{2}{c}{\shortstack{\textbf{Strict \&} \\ \textbf{RL pass}}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
 & \textbf{Chars} & \textbf{Lines} & \textbf{Chars} & \textbf{Lines} & \textbf{Chars} & \textbf{Lines} & \textbf{Chars} & \textbf{Lines} \\
\midrule
\multicolumn{9}{@{}l}{\textbf{\qwen}} \\
\quad \baselabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-qwen-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-qwen-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-qwen-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-qwen-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-qwen-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-qwen-lev-line}} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-qwen-base-mean-char}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-qwen-prompt-mean-char}}\UseMacro{fig-verl-lev-base-strict-rustfmt-qwen-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-qwen-base-mean-line}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-qwen-prompt-mean-line}}\UseMacro{fig-verl-lev-base-strict-rustfmt-qwen-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-qwen-base-mean-char}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-qwen-rl-mean-char}}\UseMacro{fig-verl-lev-both-pass-rustfmt-qwen-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-qwen-base-mean-line}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-qwen-rl-mean-line}}\UseMacro{fig-verl-lev-both-pass-rustfmt-qwen-small} & -- & -- \\
\quad \strictlabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-qwen-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-qwen-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-qwen-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-qwen-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-qwen-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-qwen-lev-line}} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-qwen-prompt-mean-char}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-qwen-base-mean-char}}\UseMacro{fig-verl-lev-base-strict-rustfmt-qwen-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-qwen-prompt-mean-line}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-qwen-base-mean-line}}\UseMacro{fig-verl-lev-base-strict-rustfmt-qwen-small} & -- & -- & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-qwen-prompt-mean-char}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-qwen-rl-mean-char}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-qwen-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-qwen-prompt-mean-line}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-qwen-rl-mean-line}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-qwen-small} \\
\quad \rllabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-qwen-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-qwen-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-qwen-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-qwen-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-qwen-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-qwen-lev-line}} & -- & -- & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-qwen-rl-mean-char}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-qwen-base-mean-char}}\UseMacro{fig-verl-lev-both-pass-rustfmt-qwen-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-qwen-rl-mean-line}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-qwen-base-mean-line}}\UseMacro{fig-verl-lev-both-pass-rustfmt-qwen-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-qwen-rl-mean-char}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-qwen-prompt-mean-char}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-qwen-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-qwen-rl-mean-line}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-qwen-prompt-mean-line}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-qwen-small} \\
\midrule
\multicolumn{9}{@{}l}{\textbf{\gpto}} \\
\quad \baselabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-gpt-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-gpt-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-gpt-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-gpt-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-gpt-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-gpt-lev-line}} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-gpt-base-mean-char}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-gpt-prompt-mean-char}}\UseMacro{fig-verl-lev-base-strict-rustfmt-gpt-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-gpt-base-mean-line}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-gpt-prompt-mean-line}}\UseMacro{fig-verl-lev-base-strict-rustfmt-gpt-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-gpt-base-mean-char}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-gpt-rl-mean-char}}\UseMacro{fig-verl-lev-both-pass-rustfmt-gpt-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-gpt-base-mean-line}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-gpt-rl-mean-line}}\UseMacro{fig-verl-lev-both-pass-rustfmt-gpt-small} & -- & -- \\
\quad \strictlabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-gpt-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-gpt-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-gpt-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-gpt-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-gpt-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-gpt-lev-line}} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-gpt-prompt-mean-char}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-gpt-base-mean-char}}\UseMacro{fig-verl-lev-base-strict-rustfmt-gpt-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-gpt-prompt-mean-line}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-gpt-base-mean-line}}\UseMacro{fig-verl-lev-base-strict-rustfmt-gpt-small} & -- & -- & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-gpt-prompt-mean-char}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-gpt-rl-mean-char}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-gpt-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-gpt-prompt-mean-line}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-gpt-rl-mean-line}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-gpt-small} \\
\quad \rllabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-gpt-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-gpt-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-gpt-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-gpt-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-gpt-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-gpt-lev-line}} & -- & -- & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-gpt-rl-mean-char}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-gpt-base-mean-char}}\UseMacro{fig-verl-lev-both-pass-rustfmt-gpt-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-gpt-rl-mean-line}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-gpt-base-mean-line}}\UseMacro{fig-verl-lev-both-pass-rustfmt-gpt-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-gpt-rl-mean-char}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-gpt-prompt-mean-char}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-gpt-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-gpt-rl-mean-line}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-gpt-prompt-mean-line}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-gpt-small} \\
\midrule
\multicolumn{9}{@{}l}{\textbf{\olmos}} \\
\quad \baselabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-olmo7b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-olmo7b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-olmo7b-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-olmo7b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-olmo7b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-olmo7b-lev-line}} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo7b-base-mean-char}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo7b-prompt-mean-char}}\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo7b-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo7b-base-mean-line}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo7b-prompt-mean-line}}\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo7b-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo7b-base-mean-char}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo7b-rl-mean-char}}\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo7b-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo7b-base-mean-line}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo7b-rl-mean-line}}\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo7b-small} & -- & -- \\
\quad \strictlabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-olmo7b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-olmo7b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-olmo7b-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-olmo7b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-olmo7b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-olmo7b-lev-line}} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo7b-prompt-mean-char}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo7b-base-mean-char}}\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo7b-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo7b-prompt-mean-line}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo7b-base-mean-line}}\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo7b-small} & -- & -- & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo7b-prompt-mean-char}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo7b-rl-mean-char}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo7b-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo7b-prompt-mean-line}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo7b-rl-mean-line}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo7b-small} \\
\quad \rllabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-olmo7b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-olmo7b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-olmo7b-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-olmo7b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-olmo7b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-olmo7b-lev-line}} & -- & -- & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo7b-rl-mean-char}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo7b-base-mean-char}}\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo7b-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo7b-rl-mean-line}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo7b-base-mean-line}}\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo7b-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo7b-rl-mean-char}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo7b-prompt-mean-char}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo7b-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo7b-rl-mean-line}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo7b-prompt-mean-line}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo7b-small} \\
\midrule
\multicolumn{9}{@{}l}{\textbf{\olmol}} \\
\quad \baselabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-olmo32b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-olmo32b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-olmo32b-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-olmo32b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-olmo32b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-olmo32b-lev-line}} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo32b-base-mean-char}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo32b-prompt-mean-char}}\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo32b-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo32b-base-mean-line}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo32b-prompt-mean-line}}\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo32b-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo32b-base-mean-char}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo32b-rl-mean-char}}\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo32b-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo32b-base-mean-line}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo32b-rl-mean-line}}\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo32b-small} & -- & -- \\
\quad \strictlabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-olmo32b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-olmo32b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-olmo32b-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-olmo32b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-olmo32b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-olmo32b-lev-line}} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo32b-prompt-mean-char}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo32b-base-mean-char}}\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo32b-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo32b-prompt-mean-line}}{\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo32b-base-mean-line}}\UseMacro{fig-verl-lev-base-strict-rustfmt-olmo32b-small} & -- & -- & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo32b-prompt-mean-char}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo32b-rl-mean-char}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo32b-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo32b-prompt-mean-line}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo32b-rl-mean-line}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo32b-small} \\
\quad \rllabel & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-olmo32b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-olmo32b-lev-char}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-olmo32b-lev-char}} & \SmallestBoldSafe{\UseMacro{fig-verl-comparison-allmean-rustfmt-verl-step62-olmo32b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-base-olmo32b-lev-line}}{\UseMacro{fig-verl-comparison-allmean-rustfmt-prompt-olmo32b-lev-line}} & -- & -- & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo32b-rl-mean-char}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo32b-base-mean-char}}\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo32b-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo32b-rl-mean-line}}{\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo32b-base-mean-line}}\UseMacro{fig-verl-lev-both-pass-rustfmt-olmo32b-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo32b-rl-mean-char}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo32b-prompt-mean-char}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo32b-small} & \SmallerBoldSafe{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo32b-rl-mean-line}}{\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo32b-prompt-mean-line}}\UseMacro{fig-verl-lev-prompt-pass-rustfmt-olmo32b-small} \\
\bottomrule
\end{tabular}
\caption{\UseMacro{TCap-verl-lev-raw-rustfmt-eval-rust-repos}}
\label{tab:verl-lev-raw-rustfmt-eval-rust-repos}
\end{table*}


==> tables/verl_meantest_nochange_table.tex <==
\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l c c c}
\toprule
\shortstack[l]{\textbf{Implementor} \\ \quad\textbf{Editor}} & \UseMacro{TCol-meantest} & \UseMacro{TCol-meantest-nc} & \UseMacro{TCol-meantest-wc} \\
\midrule
\multicolumn{4}{@{}l}{\textbf{\qwen}} \\
\quad \baselabel & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-base-qwen-mean-tests}}{\UseMacro{fig-verl-meantestnc-prompt-qwen-mean-tests}}{\UseMacro{fig-verl-meantestnc-verl-step62-qwen-mean-tests}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-base-qwen-no-change}}{\UseMacro{fig-verl-meantestnc-prompt-qwen-no-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-qwen-no-change}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-base-qwen-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-prompt-qwen-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-qwen-mean-tests-change}} \\
\quad \strictlabel & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-prompt-qwen-mean-tests}}{\UseMacro{fig-verl-meantestnc-base-qwen-mean-tests}}{\UseMacro{fig-verl-meantestnc-verl-step62-qwen-mean-tests}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-prompt-qwen-no-change}}{\UseMacro{fig-verl-meantestnc-base-qwen-no-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-qwen-no-change}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-prompt-qwen-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-base-qwen-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-qwen-mean-tests-change}} \\
\quad \rllabel & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-verl-step62-qwen-mean-tests}}{\UseMacro{fig-verl-meantestnc-base-qwen-mean-tests}}{\UseMacro{fig-verl-meantestnc-prompt-qwen-mean-tests}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-verl-step62-qwen-no-change}}{\UseMacro{fig-verl-meantestnc-base-qwen-no-change}}{\UseMacro{fig-verl-meantestnc-prompt-qwen-no-change}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-verl-step62-qwen-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-base-qwen-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-prompt-qwen-mean-tests-change}} \\
\midrule
\multicolumn{4}{@{}l}{\textbf{\gpto}} \\
\quad \baselabel & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-base-gpt-mean-tests}}{\UseMacro{fig-verl-meantestnc-prompt-gpt-mean-tests}}{\UseMacro{fig-verl-meantestnc-verl-step62-gpt-mean-tests}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-base-gpt-no-change}}{\UseMacro{fig-verl-meantestnc-prompt-gpt-no-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-gpt-no-change}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-base-gpt-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-prompt-gpt-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-gpt-mean-tests-change}} \\
\quad \strictlabel & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-prompt-gpt-mean-tests}}{\UseMacro{fig-verl-meantestnc-base-gpt-mean-tests}}{\UseMacro{fig-verl-meantestnc-verl-step62-gpt-mean-tests}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-prompt-gpt-no-change}}{\UseMacro{fig-verl-meantestnc-base-gpt-no-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-gpt-no-change}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-prompt-gpt-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-base-gpt-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-gpt-mean-tests-change}} \\
\quad \rllabel & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-verl-step62-gpt-mean-tests}}{\UseMacro{fig-verl-meantestnc-base-gpt-mean-tests}}{\UseMacro{fig-verl-meantestnc-prompt-gpt-mean-tests}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-verl-step62-gpt-no-change}}{\UseMacro{fig-verl-meantestnc-base-gpt-no-change}}{\UseMacro{fig-verl-meantestnc-prompt-gpt-no-change}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-verl-step62-gpt-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-base-gpt-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-prompt-gpt-mean-tests-change}} \\
\midrule
\multicolumn{4}{@{}l}{\textbf{\olmos}} \\
\quad \baselabel & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-base-olmo7b-mean-tests}}{\UseMacro{fig-verl-meantestnc-prompt-olmo7b-mean-tests}}{\UseMacro{fig-verl-meantestnc-verl-step62-olmo7b-mean-tests}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-base-olmo7b-no-change}}{\UseMacro{fig-verl-meantestnc-prompt-olmo7b-no-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-olmo7b-no-change}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-base-olmo7b-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-prompt-olmo7b-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-olmo7b-mean-tests-change}} \\
\quad \strictlabel & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-prompt-olmo7b-mean-tests}}{\UseMacro{fig-verl-meantestnc-base-olmo7b-mean-tests}}{\UseMacro{fig-verl-meantestnc-verl-step62-olmo7b-mean-tests}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-prompt-olmo7b-no-change}}{\UseMacro{fig-verl-meantestnc-base-olmo7b-no-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-olmo7b-no-change}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-prompt-olmo7b-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-base-olmo7b-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-olmo7b-mean-tests-change}} \\
\quad \rllabel & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-verl-step62-olmo7b-mean-tests}}{\UseMacro{fig-verl-meantestnc-base-olmo7b-mean-tests}}{\UseMacro{fig-verl-meantestnc-prompt-olmo7b-mean-tests}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-verl-step62-olmo7b-no-change}}{\UseMacro{fig-verl-meantestnc-base-olmo7b-no-change}}{\UseMacro{fig-verl-meantestnc-prompt-olmo7b-no-change}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-verl-step62-olmo7b-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-base-olmo7b-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-prompt-olmo7b-mean-tests-change}} \\
\midrule
\multicolumn{4}{@{}l}{\textbf{\olmol}} \\
\quad \baselabel & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-base-olmo32b-mean-tests}}{\UseMacro{fig-verl-meantestnc-prompt-olmo32b-mean-tests}}{\UseMacro{fig-verl-meantestnc-verl-step62-olmo32b-mean-tests}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-base-olmo32b-no-change}}{\UseMacro{fig-verl-meantestnc-prompt-olmo32b-no-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-olmo32b-no-change}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-base-olmo32b-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-prompt-olmo32b-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-olmo32b-mean-tests-change}} \\
\quad \strictlabel & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-prompt-olmo32b-mean-tests}}{\UseMacro{fig-verl-meantestnc-base-olmo32b-mean-tests}}{\UseMacro{fig-verl-meantestnc-verl-step62-olmo32b-mean-tests}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-prompt-olmo32b-no-change}}{\UseMacro{fig-verl-meantestnc-base-olmo32b-no-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-olmo32b-no-change}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-prompt-olmo32b-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-base-olmo32b-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-olmo32b-mean-tests-change}} \\
\quad \rllabel & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-verl-step62-olmo32b-mean-tests}}{\UseMacro{fig-verl-meantestnc-base-olmo32b-mean-tests}}{\UseMacro{fig-verl-meantestnc-prompt-olmo32b-mean-tests}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-verl-step62-olmo32b-no-change}}{\UseMacro{fig-verl-meantestnc-base-olmo32b-no-change}}{\UseMacro{fig-verl-meantestnc-prompt-olmo32b-no-change}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-verl-step62-olmo32b-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-base-olmo32b-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-prompt-olmo32b-mean-tests-change}} \\
\midrule
\multicolumn{4}{@{}l}{\textbf{\haiku}} \\
\quad \baselabel & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-base-haiku-mean-tests}}{\UseMacro{fig-verl-meantestnc-prompt-haiku-mean-tests}}{\UseMacro{fig-verl-meantestnc-verl-step62-haiku-mean-tests}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-base-haiku-no-change}}{\UseMacro{fig-verl-meantestnc-prompt-haiku-no-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-haiku-no-change}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-base-haiku-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-prompt-haiku-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-haiku-mean-tests-change}} \\
\quad \strictlabel & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-prompt-haiku-mean-tests}}{\UseMacro{fig-verl-meantestnc-base-haiku-mean-tests}}{\UseMacro{fig-verl-meantestnc-verl-step62-haiku-mean-tests}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-prompt-haiku-no-change}}{\UseMacro{fig-verl-meantestnc-base-haiku-no-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-haiku-no-change}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-prompt-haiku-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-base-haiku-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-verl-step62-haiku-mean-tests-change}} \\
\quad \rllabel & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-verl-step62-haiku-mean-tests}}{\UseMacro{fig-verl-meantestnc-base-haiku-mean-tests}}{\UseMacro{fig-verl-meantestnc-prompt-haiku-mean-tests}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-verl-step62-haiku-no-change}}{\UseMacro{fig-verl-meantestnc-base-haiku-no-change}}{\UseMacro{fig-verl-meantestnc-prompt-haiku-no-change}} & \LargestBoldSafe{\UseMacro{fig-verl-meantestnc-verl-step62-haiku-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-base-haiku-mean-tests-change}}{\UseMacro{fig-verl-meantestnc-prompt-haiku-mean-tests-change}} \\
\bottomrule
\end{tabular}
\caption{\UseMacro{TCap-verl-meantestnc-eval-rust-repos}}
\label{tab:verl-meantestnc-eval-rust-repos}
\end{table}
